Improved Screen Content Coding in VVC Using Soft Context Formation

Screen content images typically contain a mix of natural and synthetic image parts. Synthetic sections usually are comprised of uniformly colored areas and repeating colors and patterns. In the VVC standard, these properties are exploited using Intra Block Copy and Palette Mode. In this paper, we show that pixel-wise lossless coding can outperform lossy VVC coding in such areas. We propose an enhanced VVC coding approach for screen content images using the principle of soft context formation. First, the image is separated into two layers in a block-wise manner using a learning-based method with four block features. Synthetic image parts are coded losslessly using soft context formation, the rest with VVC.We modify the available soft context formation coder to incorporate information gained by the decoded VVC layer for improved coding efficiency. Using this approach, we achieve Bjontegaard-Delta-rate gains of 4.98% on the evaluated data sets compared to VVC.

==> Tables/blockinfo.tex <==
%\begin{tabular}{|c||c|c|c|c|}
%\hline
%QP                           & 22   & 27   & 32   & 37   \\ \hline \hline
%$r_{\mathrm{SCF}}<r_{\mathrm{VVC}}  $    & 3386 & 2984 & 2669 & 2366 \\
%$r_{\mathrm{SCF}} \geq r_{\mathrm{VVC}}$  & 3461 & 3863 & 4178 & 4481 \\ \hline
%Total                        & 6847 & 6847 & 6847 & 6847 \\ \hline
%\end{tabular}

\begin{tabular}{|c||c|c|c|c|}
\hline
QP                           & 22   & 27   & 32   & 37   \\ \hline \hline
$r_{\mathrm{SCF}}<r_{\mathrm{VVC}}  $    & 49.5~\% & 43.6~\% & 39.0~\% & 35.6~\% \\
$r_{\mathrm{SCF}} \geq r_{\mathrm{VVC}}$  & 50.5~\% & 56.4~\% & 61.0~\% & 65.4~\% \\ \hline
Total (6847 blocks)                       & 100~\% & 100~\% & 100~\% & 100~\% \\ \hline
\end{tabular}
